Language Guided Exploration for RL Agents in Text Environments

Real-world sequential decision making is characterized by sparse rewards and large decision spaces, posing significant difficulty for experiential learning systems like $\textit{tabula rasa}$ reinforcement learning (RL) agents. Large Language Models (LLMs), with a wealth of world knowledge, can help RL agents learn quickly and adapt to distribution shifts. In this work, we introduce Language Guided Exploration (LGE) framework, which uses a pre-trained language model (called GUIDE ) to provide decision-level guidance to an RL agent (called EXPLORER). We observe that on ScienceWorld (Wang et al.,2022), a challenging text environment, LGE outperforms vanilla RL agents significantly and also outperforms other sophisticated methods like Behaviour Cloning and Text Decision Transformer.

==> tables/algo_compact.tex <==
\subsubsection{Training the \textsc{Explorer}}
\begin{algorithm*}[]
\caption{Training Algorithm: \textsc{Language Guided Exploration Framework}}
\label{alg:lge_algorithm}
\begin{algorithmic}
\State Initialize replay memory $D$ to capacity $C$
\State Initialize Explorer's Q-network with random weights $\theta$
\State Initialize $update\_frequency$, $total\_steps$
\For{episode $= 1$ to $M$}
    \State env, $v$, $d$ = sample\_random\_env('train', $T$)
    \State Sample initial state $s_1$ from $d_{0}$ and get $A_{valid, 1}$ 
    \For{$t = 1$ to $N$}
        \State $total\_steps += 1$
        \State Identify $k$ most relevant actions using Guide:
        \State $\hat{A}_{relevant, t} = \text{Guide.top\_k}(A_{valid, t}, k, d_{T, v})$
        \State $random\_number \sim \text{Uniform}(0, 1)$
        \If{$random\_number > \epsilon$}
            \State $a_t \sim \text{Multinomial}(\text{softmax}(\{Q(s_t, a | \theta)$
            \State $\quad\quad\quad\quad\quad\quad\quad\text{for } a \in \hat{A}_{relevant, t}\}))$
        \Else
            \State $a_t \sim \text{Multinomial}(\text{softmax}(\{Q(s_t, a | \theta)$
            \State $\quad\quad\quad\quad\quad\quad\quad\text{for } a \in \hat{A}_{valid, t}\}))$
        \EndIf
        \State Execute $a_t$, observe $r_{t+1}$, $s_{t+1}$, $A_{valid, t+1}$
        \State Store $(s_t, a_t, r_{t+1}, s_{t+1}, A_{valid, t+1})$ in $D$
        \If{$total\_steps$ \% $update\_frequency = 0$}
            \State Sample batch from $D$
            \State $L_{\text{cumulative}} = 0$
            \For{each $(s, a, r, s', A')$ in batch}
                \State $\delta = r + \gamma \max_{a' \in A'} Q(s', a'| \theta) $
                \State $\quad\quad  - Q(s, a| \theta)$
                \State Compute Huber loss: 
                \State $L = \begin{cases} 
                  \frac{1}{2} \delta^2 & \text{if } |\delta| < 1 \\
                  |\delta| - \frac{1}{2} & \text{otherwise}
               \end{cases}$
                \State $L_{\text{cumulative}} += L$
            \EndFor
            \State Update $\theta$ with Adam optimizer:
            \State $\theta \leftarrow \text{AdamOptimizer}(\theta, \nabla_{\theta} L_{\text{cumulative}})$
        \EndIf
        \State Update state: $s_t \leftarrow s_{t+1}$
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm*}


==> tables/evaluating_guide_ranking.tex <==
\begin{table}[]
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Metric}      & \textbf{Value}   \\ \midrule
Avg. GAR             & $7.42 \pm 16.23$ \\
Avg. GAR (\%)        & $1.85 \pm 9.42$  \\
Avg. GARR                 & $0.31$           \\
Avg. $|A_{\text{val},t}|$ & $1908 \pm 1660$  \\ \bottomrule
\end{tabular}%
%}
\caption{Evaluating Guide's ability to Rank}
\label{tab:Guide gold ranks}
\end{table}

==> tables/evaluating_guide_set.tex <==
\begin{table}[]
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Model}                  & \textbf{top-k} & \textbf{RSR} & \textbf{MAP} \\ \midrule
Gold Global                     & 50             & 0.71            & 0.52                    \\
Gold per-task                   & 50             & 0.9             & 0.66                    \\ \midrule
\multirow{4}{*}{\textsc{Guide}} & 50             & 0.99            & 0.68                    \\
                                & 20             & 0.94            & 0.67                    \\
                                & 10             & 0.79            & 0.61                    \\ \bottomrule
                                %& 5              & 0.57            & 0.49                    \\ \bottomrule
\end{tabular}%
%}
\caption{Evaluating Guide's ability to extract relevant actions}
\label{tab:Evaluating Guide by set based metric}
\end{table}

==> tables/main_table_long.tex <==
\begin{table*}[!t]
    %\rowcolors{2}{gray!100}{white}
\centering
\scriptsize
\vspace{8mm}
\begin{tabular}{lcccccccc}
% \textbf{\#} & \textbf{Topic} & \textbf{Task} &
 \textbf{Task Description} & Random-Valid & DRRN & KG-A2C & CALM & BC & TDT & LGE ($\epsilon_{inc}$) & LGE ($\epsilon_{fixed}$) \\
%\begin{rotate}{0} Random-Valid \end{rotate} &
%\begin{rotate}{0} DRRN \end{rotate} &
%\begin{rotate}{0} KG-A2C \end{rotate} &
%\begin{rotate}{0} CALM \end{rotate} &
%\begin{rotate}{0} BC \end{rotate} &
%\begin{rotate}{0} TDT \end{rotate} \\[1mm] 
%\vspace{-2mm}
%~\\[1pt]
%Model                                   &   Det     &  Z1       &   Z3      &   OMNI    &  ENCH     &   SPIR    &       &   \\[1mm]
\toprule
     \multicolumn{1}{l}{\textbf{Test Time Valid Action Detection Aid}}  &                   $\checkmark$                 & $\checkmark$      &     &   &   $\checkmark$  & $\checkmark$         &    $\checkmark$ & 
     $\checkmark$  \\

\toprule
\rowcolor[HTML]{D3D3D3} 
% 1-1  & Matter         &
Changes of State (Boiling)                  & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.04 & 0.02 \\ % Task 0
\rowcolor[HTML]{D3D3D3} 
% 1-2  & Matter         & 
Changes of State (Melting)                  & 0.00 & 0.04 & 0.00 & 0.00 & 0.00 & 0.01 & 0.02 & 0.03 \\ % Task 3
\rowcolor[HTML]{D3D3D3} 
% 1-3  & Matter         & 
Changes of State (Freezing)                 & 0.00 & 0.01 & 0.04 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 \\ % Task 2
\rowcolor[HTML]{D3D3D3} 
% 1-4  & Matter         & 
Changes of State (Any)                      & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.03 \\ \hline  % Task 1
% 2-1  & Measurement &
Use Thermometer                             & 0.00 & 0.10 & 0.06 & 0.01 & 0.04 & 0.04 & 0.08 & 0.11 \\ % Task 6
% 2-2  & Measurement    & 
Measuring Boiling Point (known)             & 0.00 & 0.08 & 0.11 & 0.01 & 0.01 & 0.02 & 0.08 & 0.08\\ % Task 4
% 2-3  & Measurement    & 
Measuring Boiling Point (unknown)           & 0.00 & 0.06 & 0.04 & 0.01 & 0.01 & 0.02 & 0.06 & 0.07 \\ \hline % Task 5
\rowcolor[HTML]{D3D3D3} 
% 3-1  & Electricity    & 
Create a circuit                            & 0.01 & 0.13 & 0.07 & 0.05 & 0.03 & 0.07 & 0.13 & 0.13 \\ % Task 7
\rowcolor[HTML]{D3D3D3} 
% 3-2  & Electricity    & 
Renewable vs Non-renewable Energy           & 0.01 & 0.10 & 0.04 & 0.07 & 0.02 & 0.05 & 0.08 & 0.1 \\ % Task 8
\rowcolor[HTML]{D3D3D3} 
% 3-3  & Electricity    & 
Test Conductivity (known)                   & 0.01 & 0.07 & 0.04 & 0.02 & 0.05 & 0.05 & 0.06 & 0.06 \\ % Task 9
\rowcolor[HTML]{D3D3D3} 
% 3-4  & Electricity    & 
Test Conductivity (unknown)                 & 0.00 & 0.20 & 0.04 & 0.02 & 0.04 & 0.05 & 0.23 & 0.29 \\ \hline % Task 10
% 4-1  & Classification & 
Find a living thing                         & 0.03 & 0.26 & 0.18 & 0.10 & 0.29 & 0.16 & 0.18 & 0.56 \\ % Task 12
% 4-2  & Classification & 
Find a non-living thing                     & 0.63 & 0.56 & 0.44 & 0.54 & 0.19 & 0.17 & 0.55 & 0.60 \\ % Task 13
% 4-3  & Classification & 
Find a plant                                & 0.01 & 0.19 & 0.16 & 0.10 & 0.17 & 0.19 & 0.19 & 0.67 \\ % Task 14
% 4-4  & Classification & 
Find an animal                              & 0.01 & 0.19 & 0.15 & 0.08 & 0.21 & 0.19 & 0.39 & 0.19 \\ \hline % Task 11
\rowcolor[HTML]{D3D3D3} 
% 5-1  & Biology        & 
Grow a plant                                & 0.07 & 0.09 & 0.06 & 0.02 & 0.08 & 0.03 & 0.10 & 0.094 \\ % Task 16
\rowcolor[HTML]{D3D3D3} 
% 5-2  & Biology        & 
Grow a fruit                                & 0.02 & 0.16 & 0.11 & 0.04 & 0.03 & 0.05 & 0.18 & 0.17 \\ \hline % Task 15
% 6-1  & Chemistry      & 
Mixing (generic)                            & 0.01 & 0.20 & 0.17 & 0.03 & 0.06 & 0.10 & 0.21 & 0.25 \\ % Task 17
% 6-2  & Chemistry      & 
Mixing paints (secondary colours)           & 0.01 & 0.29 & 0.19 & 0.06 & 0.16 & 0.20 & 0.30 & 0.27 \\ % Task 18
% 6-3  & Chemistry      & 
Mixing paints (tertiary colours)            & 0.00 & 0.11 & 0.04 & 0.03 & 0.05 & 0.07 & 0.11 & 0.11 \\ \hline % Task 19
\rowcolor[HTML]{D3D3D3} 
% 7-1  & Biology        & 
Identify longest-lived animal               & 0.02 & 0.48 & 0.43 & 0.06 & 0.26 & 0.20 & 0.55 & 0.89 \\ % Task 20
\rowcolor[HTML]{D3D3D3} 
% 7-2  & Biology        & 
Identify shortest-lived animal              & 0.03 & 0.47 & 0.32 & 0.10 & 0.14 & 0.16 & 0.64 & 0.46 \\ % Task 22
\rowcolor[HTML]{D3D3D3} 
% 7-3  & Biology        & 
Identify longest-then-shortest-lived animal & 0.01 & 0.31 & 0.23 & 0.04 & 0.02 & 0.20 & 0.33 & 0.32 \\ \hline % Task 21
% 8-1  & Biology        & 
Identify life stages (plant)                & 0.00 & 0.09 & 0.05 & 0.04 & 0.04 & 0.02 & 0.16 & 0.05 \\ % Task 24
% 8-2  & Biology        & 
Identify life stages (animal)               & 0.00 & 0.10 & 0.10 & 0.00 & 0.02 & 0.07 & 0.17 & 0.18 \\ \hline % Task 23
\rowcolor[HTML]{D3D3D3} 
% 9-1  & Forces         & 
Inclined Planes (determine angle)           & 0.01 & 0.13 & 0.04 & 0.00 & 0.05 & 0.04 & 0.24 & 0.25\\ % Task 25
\rowcolor[HTML]{D3D3D3} 
% 9-2  & Forces         & 
Friction (known surfaces)                   & 0.00 & 0.13 & 0.04 & 0.03 & 0.05 & 0.04 & 0.25 & 0.24 \\ % Task 26
\rowcolor[HTML]{D3D3D3} 
% 9-3  & Forces         & 
Friction (unknown surfaces)                 & 0.01 & 0.13 & 0.04 & 0.02 & 0.04 & 0.04 & 0.21 & 0.21 \\ \hline % Task 27
% 10-1 & Biology        & 
Mendelian Genetics (known plants)           & 0.01 & 0.19 & 0.11 & 0.02 & 0.06 & 0.06 & 0.19 & 0.22 \\ % Task 28
% 10-2 & Biology        & 
Mendelian Genetics (unknown plants)         & 0.01 & 0.17 & 0.11 & 0.02 & 0.13 & 0.05 & 0.17 & 0.16 \\ % Task 29
\midrule
     \multicolumn{1}{l}{\textbf{Average}}                                     & {0.03}      &   {0.17}  &       {0.11}  &   {0.05}  &   {0.08}  &   {0.08} & {0.20} & \textbf{0.23}\\
        % \multicolumn{2}{l}{\textbf{Param. Count $\times10^6$}}  &                                   &  --    &  \textbf{1.5}   &    5.5     &  131\textsuperscript{*}   &   11,000  & 11,000  \\
\bottomrule
\end{tabular}
\caption{\footnotesize Zero-shot performance of the agents on test variations of across all tasks.}%\todo{(explain known vs unknown variations in caption too)}}
\label{tab:agent-performance} 
%\vspace{-4mm}
\end{table*}

